Toward Efficient Generalization in 3D Human Pose Estimation via a Canonical Domain Approach

Recent advancements in deep learning methods have significantly improved the performance of 3D Human Pose Estimation (HPE). However, performance degradation caused by domain gaps between source and target domains remains a major challenge to generalization, necessitating extensive data augmentation and/or fine-tuning for each specific target domain. To address this issue more efficiently, we propose a novel canonical domain approach that maps both the source and target domains into a unified canonical domain, alleviating the need for additional fine-tuning in the target domain. To construct the canonical domain, we introduce a canonicalization process to generate a novel canonical 2D-3D pose mapping that ensures 2D-3D pose consistency and simplifies 2D-3D pose patterns, enabling more efficient training of lifting networks. The canonicalization of both domains is achieved through the following steps: (1) in the source domain, the lifting network is trained within the canonical domain; (2) in the target domain, input 2D poses are canonicalized prior to inference by leveraging the properties of perspective projection and known camera intrinsics. Consequently, the trained network can be directly applied to the target domain without requiring additional fine-tuning. Experiments conducted with various lifting networks and publicly available datasets (e.g., Human3.6M, Fit3D, MPI-INF-3DHP) demonstrate that the proposed method substantially improves generalization capability across datasets while using the same data volume.

==> sec/9_biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{ACCESS_latex_template_202303/images/Hoosang.jpg}}]{Hoosang Lee} received his B.S. degree in robotics from Kwangwoon University, Seoul, South Korea, in 2018, and his M.S. degree in intelligent robotics technology from the Gwangju Institute of Science and Technology (GIST), Gwangju, South Korea, in 2020. He is currently pursuing a Ph.D. in intelligent robotics technology at the School of Integrated Technology. His research interests include deep learning-based computer vision and robotic control.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{ACCESS_latex_template_202303/images/Jeha.jpg}}]{Jeha Ryu} received his B.S. degree in Mechanical Engineering from Seoul National University, Seoul, South Korea, in 1982, his M.S. degree in Mechanical Engineering from the Korea Advanced Institute of Science and Technology (KAIST), Daejeon, South Korea, in 1984, and his Ph.D. degree in Mechanical Engineering from The University of Iowa, Iowa City, IA, USA, in 1991. He has served as a professor at the School of Mechatronics, the School of Integrated Technology, and the Artificial Intelligence Graduate School at the Gwangju Institute of Science and Technology (GIST), Gwangju, South Korea. Currently, he holds the position of Emeritus Professor at the School of Integrated Technology. Prof. Ryu has published more than 300 research articles and reports. His research interests span both fundamental and applied research in artificial intelligence, particularly its applications in diverse fields such as medical and rehabilitation robotics, autonomous vehicles, teleoperation, haptics, virtual reality, and augmented reality. His current focus includes intelligent robot controls and image processing using artificial intelligence. He is a member of KROS, KSAE, ICROS, and KSME.
\end{IEEEbiography}


